Improving the Transferability of Adversarial Attacks by an Input Transpose

Deep neural networks (DNNs) are highly susceptible to adversarial examples--subtle perturbations applied to inputs that are often imperceptible to humans yet lead to incorrect model predictions. In black-box scenarios, however, existing adversarial examples exhibit limited transferability and struggle to effectively compromise multiple unseen DNN models. Previous strategies enhance the cross-model generalization of adversarial examples by introducing versatility into adversarial perturbations, thereby improving transferability. However, further refining perturbation versatility often demands intricate algorithm development and substantial computation consumption. In this work, we propose an input transpose method that requires almost no additional labor and computation costs but can significantly improve the transferability of existing adversarial strategies. Even without adding adversarial perturbations, our method demonstrates considerable effectiveness in cross-model attacks. Our exploration finds that on specific datasets, a mere $1^\circ$ left or right rotation might be sufficient for most adversarial examples to deceive unseen models. Our further analysis suggests that this transferability improvement triggered by rotating only $1^\circ$ may stem from visible pattern shifts in the DNN's low-level feature maps. Moreover, this transferability exhibits optimal angles that, when identified under unrestricted query conditions, could potentially yield even greater performance.

==> sec/5_discuss.tex <==
\section{Discussion}
While our method achieves substantial improvements in transferability, we observed a minor, unexpected behavior: on certain white-box scenarios, specifically one of the seven baseline attacks, our method occasionally shows slightly reduced effectiveness. Please see our supplementary. This phenomenon appears limited in scope and does not affect the overall robustness of our approach in adversarial transferability since we mainly focus on the cross-model capability of AEs. We view this as an opportunity for further refinement and plan to address it in future work to ensure consistently high performance across all scenarios.
